Learning and Certification under Instance-targeted Poisoning

In this paper, we study PAC learnability and certification of predictions under instance-targeted poisoning attacks, where the adversary who knows the test instance may change a fraction of the training set with the goal of fooling the learner at the test instance. Our first contribution is to formalize the problem in various settings and to explicitly model subtle aspects such as the proper or improper nature of the learning, learner's randomness, and whether (or not) adversary's attack can depend on it. Our main result shows that when the budget of the adversary scales sublinearly with the sample complexity, (improper) PAC learnability and certification are achievable; in contrast, when the adversary's budget grows linearly with the sample complexity, the adversary can potentially drive up the expected 0-1 loss to one. We also study distribution-specific PAC learning in the same attack model and show that proper learning with certification is possible for learning half spaces under natural distributions. Finally, we empirically study the robustness of K nearest neighbour, logistic regression, multi-layer perceptron, and convolutional neural network on real data sets against targeted-poisoning attacks. Our experimental results show that many models, especially state-of-the-art neural networks, are indeed vulnerable to these strong attacks. Interestingly, we observe that methods with high standard accuracy might be more vulnerable to instance-targeted poisoning attacks.

==> AttackClasses.tex <==

\section{Other Adversarial Classes} \label{sec:attacks}
Main adversarial attacks that we envision are  the following. In each case we state the constraint that $\cS'$ has based on $\cS$.
\begin{itemize} 
    \item {\bf $\Add_b$ ($b$-adding):} the adversary adds up to $b$ examples to $\cS$ and put them in arbitrary order. Namely, the multi-set $\cS'$  has size at most $|\cS|+b$ and it holds that $\cS \se \cS'$.
    \item {\bf $\Rem_b$ ($b$-removing):} the adversary removes up to $b$ examples from $\cS$ and puts the elements in  an arbitrary order. Namely, as multi-sets $|\cS'| \geq |\cS|-b$ and   $\cS' \subseteq \cS$.


    \item {\bf $\Flp_b$ ($b$-label flipping):} the adversary changes the label of up to $b$ examples in $\cS$ and puts the final set in an arbitrary order.
\end{itemize}
For some natural measures, (all above with the exception of $b$-removing) $b$ is bounded by the sample complexity $m$. However, for $b$-adding adversaries $b$ could be bigger than $m$.  



\paragraph{Randomized  poisoning.} By default, we think of a particular adversary as a mapping (i.e., a function). Note, however, that adversarial patterns might be randomized; e.g., the $p$-tampering adversaries of \cite{mahloujifar2018learning} allow an adversary to change each  example with \emph{independent} probability $p$.


\paragraph{Computational efficiency of attacks.} The above-mentioned restrictions on adversary's budget in the amount of perturbations for $\cS$ still ignores whether the attacker runs in polynomial time or not. Indeed, the above definitions are all ``information theoretic'' and one can further restrict the adversary to run in polynomial time (e.g., with or without oracle access to sampling more data from $D$) and leverage this with the hope of improving the robustness. Whether or not this can be done is also an interesting open question for future work. We also note that computational efficiency of the attack is a different issue than the efficiency of the \emph{learner} itself, which is a focus of recent work on robust statistics with computationally tractable learners \cite{diakonikolas2016robust,lai2016agnostic}.

\paragraph{Attacks that avoid wrong labels.} One can further limit the power of an adversary in what poison points it can add to $\cS$. Let $\cH$ be a hypothesis class. Recall that a distribution $D$ over $\cX\times \cY$ is realizable if  there is some $h \in \cH$ such that $\Pr_{(x,y)\sim D}[h(x)=y]=\Pr_{(x,y)\sim \cS}[h(x)=y]=1$. We call a training set $\cS$ realizable, if the uniform distribution over $\cS$ is realizable, and we call $(D,\cS)$ jointly realizable if there is $h \in \cH$ such that $\Pr_{(x,y)\sim D}[h(x)=y]=\Pr_{(x,y)\sim \cS}[h(x)=y]=1$.
\begin{itemize}
    \item {\bf Clean-label attacks.} An adversary  $\Adv$ is \emph{clean-label} with respect to $D$, if for any training set $\cS$ that is jointly realizable with $D$, and any target point $e$,  the adversary's output set $\cS'$ is jointly realizable with $D$.
    \item {\bf Label-consistent attacks.} An adversary  $\Adv$ is \emph{label-consistent}, if for any training set $\cS$ that is  realizable, and any target point $e$,  the adversary's output set $\cS'$ is  realizable.
\end{itemize} 
Note that label-consistent attacks might \emph{not} be clean label. For example, an adversary might  substitute an entire  training set $\cS$ with a new set $\cS'$ that is consistent with some arbitrary $h' \in \cH$.


==> nontarg.tex <==
\section{Learnability under Non-targeted Poisoning} \label{sec:non-tar}

The results of this section reviews results showing that whenever the uniform convergence holds, then PAC learning of classification tasks under \emph{non-targeted} data poisoning is possible in general, if and only if the adversarial budget is $b(m)=o(m)$.
%
We first go over  the lower bound, and state a result implicit in \cite{diochnos2019lower}.

\begin{proposition}[Lower bound on PAC learning under non-targeted poisoning attacks \cite{diochnos2019lower}]
For the hypothesis class $\cH$ of homogeneous half spaces in dimension $d$ and even under the (fixed) uniform distribution over the unit sphere (in dimension $d$) a \emph{non-targeted} adversary $\AdvC_b$ who can remove $b(m)$ of the samples, for any learner, it holds that there is $h \in \cH$ such that the learner under the non-targeted attacks from $\AdvC_b$ would err by at least $\Omega(b/m)$. Hence, if $b=\Omega(m)$, the problem is not PAC learnable under such non-targeted attacks.
\end{proposition}

\begin{proof}
The proof is essentially the same as the proof of Theorem 3.4 from \cite{diochnos2019lower}, but this time we do not deal with evasion attacks.

Consider two half spaces $h,h'$ that have exactly $\beta$ measure of points falling into their disagreement region (i.e., the points on which they disagree with). Then, a poisoning adversary can delete all these $\beta$-fraction of the points from the data set (or substitute them with fixed points in the $b$-changing adversarial model). In that case, the learner would not be able to distinguish between these two models, and hence will err at least on half of the disagreement region. This leads to error $\Omega(\beta)$ by the learner on at least one of these half spaces.
\end{proof}


The  following states that the ERM (empirical risk minimizer) rule will lead to a PAC learning algorithm robust to \emph{non-targeted} poisoning adversaries who could change $o(m)$ number of examples \cite{bshouty2002pac}. The bound is also tight due to the proposition above, in the sense that if the adversary can change $b(m)=\Omega(m)=\beta \cdot m$ of the examples, there are hypothesis classes (e.g., half spaces) for which it can increase the population error up to $\Omega(\beta)=\Omega(1)$. 

\begin{proposition}
Suppose a hypothesis class $\cH$ has bounded VC dimension, and suppose a non-targeted adversary has budget $b(m)=o(m)$. Then the same hypothesis class is PAC learnable even under such  non-targeted poisoning attacks.
\end{proposition}

\begin{proof}
If $\cH$ has bounded VC dimension, then it can be learned using the ERM rule, and using the \emph{uniform} convergence argument. Namely, if there is no attack, then for every $(\eps,\delta)$, there is $m=$
hypothesis class is $(\eps,\delta)$-PAC learnable using $m=\MUC(\eps, \delta)$ such that for any distribution $D$, with probability $1-\delta$ over the training set $\cS \gets D^m$, it holds that for \emph{all} $h \in \cH$ the empirical risk and population risks are $\eps$ close; namely, $\Pr_{(x,y) \sim \cS}[h(x)\neq y] \in  \Pr_{(x,y) \sim D}[h(x)\neq y]  \pm \eps.$ 

Using this, we use the same ERM rule to prove the PAC learning even under $o(m)$ changes to the training set by the adversary. It is sufficient to prove the following lemma.

For simplicity we use the notation $\loss(h,\cS)$ to denote the empirical risk over $\cS$ and $\ell(h,D)$ to denote the population risk of $h$ under  $D$.
\begin{lemma} 
For every $\eps, \delta \in (0, 1)$ and for every distribution $D$, if $\cS$ is a sample of $m \geq \MUC(\eps, \delta)$ examples drawn i.i.d. according to $D$ and $\cS'$ is the poisoned version of $\cS$ that $\HD(\cS', \cS) \leq \beta \cdot m$, where $\HD$ is the Hamming distance\footnote{Note that even though we allow the adversary to reorder the data set after poisoning, since the ERM rule treats the data in $\cS'$ symmetrically, we can pretend that the attack is limited in the Hamming distance.} then with probability at least $1-\delta$ over the sampling of  $\cS$ we have for  $\loss(h_{\cS'},D) \leq \min_{h \in \cH}\loss(h,D) + 2\eps + 2r$ where $h_{\cS'} = \text{ERM}_{\cH}(\cS') = \argmin_{h \in \cH} \loss(h,\cS')$.
\label{lemma:pac_global_robust}
\end{lemma}
In the rest, we just have to prove this lemma. 

Let $h_{\cS} = \min_{h \in \cH}\loss(h,\cS)$. Then,

\begin{equation}
\begin{split}
    \loss(h_{\cS'},\cS) 
    & \leq \loss(h_{\cS'},\cS') + \beta \\
    & \leq \loss(h_\cS,\cS') + \beta \\
    & \leq \loss(h_\cS,\cS') + 2\beta \\
\end{split}
\end{equation}


By the uniform convergence, with probability at least $1-\delta$, we have $\cS$ is $\eps$-representative, i.e.
\begin{equation*}
     \forall h \in \cH,~~ |\loss(h,S) - \loss(h,D)| \leq \eps 
\end{equation*}

Therefore,
\begin{equation}
    \loss{(h_\cS,\cS)} \leq \loss(h,\cS) \leq \min_{h \in \cH}\loss(h,D) + \eps
\end{equation}

Similarly, 
\begin{equation}
        \loss(h_{\cS'},D) \leq \loss(h_{\cS'},\cS) + \eps
\end{equation}

Therefore, with probability at least $1 - \delta$ we have $\loss(h_{\cS'},D) \leq \min_{h \in \cH}\loss(h,D) + 2\eps + 2\beta$.

\end{proof}

Lemma \ref{lemma:pac_global_robust} shows a poisoning attack with $\beta \cdot m$ data difference can only change $\beta$ on both empirical error and generalization error of an ERM learner. However, this result is not equivalent to the instance-targeted robustness of the model, since for instance-targeted poisoning, an adversary can select the poisoning examples differently for every example. Even the algorithm is non-targeted robust, an extreme case is still possible that the adversary is able to poison every example. 


==> otherproof.tex <==
%\section{Proofs} \label{sec:proofs}










%\begin{proof}[Proof of \ref{thm:limit-agnostic}] Consider the case that for every $x \in \cX$, a label $y \in \{0, 1\}$ is randomly assigned to it. In this case, every $h \in \cH$ has a loss of $0.5$. 
% However, to change the prediction of sample $x, y$, an adversary can simply add $(x, -y)$ into the dataset. In this case the learner will always fail with high probability. \end{proof}













==> remarks.tex <==
\section{Extension and Remarks for Main Definitions} 
Here we discuss some extensions to Definitions of Section \ref{sec:Defs}. These extensions    could be combined as well, but we discuss them  by only modifying the baseline Definitions of Section \ref{sec:Defs}.


\paragraph{Other ways to be targeted (or not).} Definitions  \ref{def:TarRob} and \ref{def:TarRisk} uses the term targeted to   refer to the fact that the example $e$ is known to the adversary. Previous work \cite{shafahi2018poison, zhu2019transferable}   on poisoning attacks have studied other forms of being targeted as well, e.g., by aiming to force the learner obtain  a particular (targeted) label for the attacked instance $x$. 

On the other hand, if one does \emph{not} allow the adversary to know $e$ before choosing the poisoning pattern, then one obtains a notion of robustness (as well as certification~\cite{steinhardt2017certified}) that can still allows the adversary to pick its strategy based on $\cS$.


%\paragraph{Robustness of even wrong predictions.} Definitions \ref{def:TarRisk} and \ref{def:TarRob} define robustness and risk based on the requirement that the  prediction on $x$ using the modified training set shall flip from correct to wrong. One can also define robustness regardless of the correctness of the decision as to how many changes it takes to simply flip the decision.\footnote{The same choices can be made in the context of inference-time attacks as well; see \cite{diochnos2018adversarial} for more discussions.} However,  we only use robustness to refer to being robust for the correct prediction. When it comes to \emph{certification}, however, we will deal with cases where a certified is not sure about the label that it certifies.



%\item{\bf Other restrictions on adversaries.} Definition \ref{def:TarRobRisk} works with the total number of changes (i.e., removals followed by addition) to the training set. One can define other ways by which the adversary can change the training set. For example, we can work with \emph{removing-only} or \emph{adding-only} adversaries instead. Or, one can only allow changing the labels of the examples as is done in the previous works of \cite{rosenfeld2020certified,levine2020deep}







 \paragraph{Randomized learners.}  We now show how to extend these base definitions to the setting of randomized learners. Note that we still keep the hypothesis functions deterministic.

\remove{ 
\begin{definition}[Alternative definitions for randomized learners]  \Mnote{we probably remove the following def.}
  The definitions of Section \ref{sec:Defs} either use a \emph{worst-case} approach for handling adversarial perturbations, or for case of  randomized learners it presents a weak notion of loss and risk as well.   Here we present alternative natural definitions for the case of randomized learners. If we still pick the random seed $r$ at random but let the adversary know this, then we obtain a definition of adversarial loss that is different from those in Definition \ref{def:TarRisk}.

One can imagine stronger attacks in which the adversary somehow gets to know the randomness of the learner and crafts the set $\cS'$ based on that. To model risk and robustness for such attacks, we envision  adversaries in $\Adv$ that also take $r$ as input. Then we use $\Adv(\textcolor{red}{r},\cS,e)$ to obtain the poisoned set for definitions of $\loss_{ \AdvC}(\cS,e)$ and  $\Rob^\tau_{\AdvC}(\cS,e)$.


For weak adversaries who do not know the randomness, we can also define an average-case notion of robustness that intuitively captures the following: the robustness bound $b$ states the budget of adversary that is needed to increase the probability of wrong prediction to a specific threshold  $\tau \in [0,1]$ (e.g., $\tau=0.99$). %Then we can call a decision on point $x$ robust up to budget-$b$ attacks if with probability $\tau$ we get the same  prediction regardless of the attack, as long as learner's randomness $r$ is chosen independent of the adversary's perturbation.
    $$\Rob^{\textcolor{red}{\tau}}_{\AdvC}(\cS,e)= \min \set{b \mid \exists \Adv \in \AdvC_b, \Pr_r[\Learn_r(\Adv(\cS,e))(x)=y] < \tau}.$$


  We also can generalize the above notion of robustness for weak adversaries (against randomized learners) to the certifying regime. We call a randomized certifying learner $\Learn$  certifying for distribution $D$ with    parameter $\tau \in (0,1]$ if whenever we run $\Learn$  on i.i.d. sampled $S \sim D^m$, and if $\Learn(\cS)=h,h(x)=(y,b)$ gives the correct label for the example $(x,y) \sim D$, then the certification $b$ is valid: $\Rob^\tau_\AdvC(\cS,e) > b$. In that case, we define the certified correctness as:
 $$\CCor^{\textcolor{red}{\tau}}_{\AdvC_b}(\cS,D)=
 \Pr_{h = \Learn(\cS), (x,y) \sim D}[\hpred(x)=y \land  \hcert(x) \geq k].$$
 Allowing randomized learners, we say that a hypothesis class is \emph{certifiably} (improperly and/or agnostically) PAC learnable (using randomized learners) if there is a function $\tau(m) \in (0,1]$ where $\lim_{m \to \infty}\tau(m) =1 $ and Definition \ref{def:TarPAC} holds,  while we use $1-\CCor^{\tau(m)}_\AdvC(\cS,D)$ instead of $\Risk_\AdvC(\cS,D)$. 
 
    \end{definition}


\paragraph{Robustness for regression tasks.} One can still define the notions of robustness and certified robustness similar to how we defined them using a parameter $\tau$ above for the randomized case. Namely, the certifying predictor guarantees that if we assume the prediction $y$ is the true label, then even up to $b$ degree of perturbations to the training set that has produced this model would not lead to a model that predicts $x$ with more than $\tau$ loss.
}



==> temp.tex <==



% \section{Ensemble}



% \begin{definition}[Point-wise Robustness]

% For a model $h=\Learn(S)$, a sample $x$ is $r$-Point-wise Robust to poisoning attacks if for all $S'$ that $|S' \cup S| -|S' \cap S| \leq r|S|$ and $h' = \Learn(S')$, we have $h'(x) = c(x)$. 

% \end{definition}



% \begin{lemma}
% For a majority ensemble model $\modelensemble: \{h_1, \dots, h_t \}$, suppose $t$ is large enough and each sub-model $h_i$ is independently trained with $m$ examples that i.i.d sampled from $\cS$ with replacement and has generalization error $\epsilon$ when trained with no poisoning samples. The model $\modelensemble$ is $k$-robust correct for $(1-2(\epsilon + mk/n))n$ examples where $k \leq n/2m$. 
% \end{lemma}

% \begin{proof}

% With $k$ poisoning examples, by definition each sub-model $h_i$ has a chance of $(1-k/n)^m > 1 - mk/n$ that doesn't contain any poisoning samples. 

% For a random example $e = (x_e, y_e)$ that is drawn from $\cD$, let $\epsilon_e = \Pr[h_i(x_e) = y_e]$ indicates the error probability that a sub-model $h_i$ that predicts $e$ incorrectly. Then with $\cS'$, each $p_e$ has probability at least $(1 - \epsilon_e)(1 - mk/n)$ to correctly predicts $e$. Therefore, the probability for $\modelensemble$ to correctly predicts $e$ is $\Pr[(1 - \epsilon_e)(1 - mk/n) \geq 1/2]$.

% By the definition of generalization error, we have $\Ex_{e \sim \cD}[\epsilon_e] = \epsilon$. Therefore, by Markov's inequality we have $\Pr[\epsilon_e \geq 1 - \frac{1}{2(1 - mk/n)}] \leq \frac{2\epsilon(1 - mk/n)}{1 - 2mk/n} \leq 2\epsilon + 2mk/n$.
% \end{proof}




% \begin{proof}

% To proof the lemma, we show that majority ensemble model $\modelensemble$ is also $r$-strong-robust PAC learner 
% if every sub-model samples independently and trains with ERM rule. Suppose $\cS$ has size $n$, we hope to build a function $n = \hat{m}_\cH(\epsilon, \delta)$ to prove $\modelensemble$ is a $r$-strong-robust PAC learner.
% % For simplicity, we use $\Learn(S^m)$ to denote the distribution of models learn from $\Learn$ with $m$ i.i.d. samples from $\cS$.

% For a random example $e = (x_e, y_e)$ that is drawn from $\cD$, let $\epsilon_e = \Pr_{h \sim \Learn(\cS^m)}[h(x_e) \neq y_e]$ indicates the error probability that a random sub-model $h$, trained with original training dataset $\cS$, predicts $e$ incorrectly.
% % let $\epsilon_e = \Pr[h_i(x_e) \neq y_e]$ indicates the error probability that a sub-model $h_i$, which is trained with original training dataset $\cS$, predicts $e$ incorrectly. Then with $\cS'$, each $h_i$ has probability at least $(1 - \epsilon_e - m_1r)$ to correctly predicts $e$. 
% % Then for $\cS'$, we have $\Pr_{h \sim \Learn({\cS'}^m)}[h(x_e) = y_e] \geq (1 - m_1r  - \epsilon_e)$.

% The probability for $\modelensemble$ to correctly predict $e$ is $\Pr_{\modelensemble \sim \Learn(\cS')}[\modelensemble(x_e) = y_e] \geq \Pr_{\modelensemble \sim \Learn(\cS')}[\sum_{i=1}^T (h_i(x_e) = y_e) \geq \frac{K}{2}]$. Therefore, for a large enough $K$, if $\Pr_{h \sim \Learn({\cS'}^m)}[h(x_e) = y_e] \geq 2/3$, we have $\Pr_{\modelensemble \sim \Learn(\cS')}[\sum_{i=1}^T (h_i(x_e) = y_e) \geq \frac{K}{2}] \geq 1 - \epsilon_0$ where $\epsilon_0$ is negligible.

% By the definition of generalization error, we have $\Pr_{h \sim \Learn({\cS}^m)}[\Ex_{e \sim \cD}[\epsilon_e] \leq \epsilon_1] \geq 1 - \delta_1$ for sample $e$. For those $h$ that has $\Ex_{e \sim \cD}[\epsilon_e] \leq \epsilon_1$, by Markov's inequality we have $\Pr_{e \sim \cD}[(1 - \epsilon_e - m_1r) \leq 2/3] = \Pr_{e \sim \cD}[\epsilon_e \geq 1/3  - m_1r] \leq \frac{3\epsilon_1}{1 - 3m_1r} $. Therefore, 
% \begin{equation*}
%  \Pr_{h \sim \Learn(\cS^m)}\left[\Pr_{e \sim \cD}[(1 -\epsilon_e - m_1r) \geq 2/3  ] \geq 1 -  \frac{3\epsilon_1}{1 - 3m_1r} \right] \geq 1 - \delta_1.   
% \end{equation*}

% Therefore, $\Pr_{e \in D}[(1 - \epsilon_e - m_1r) \geq 2/3] \geq (1 - \delta_1 -  \frac{3\epsilon_1}{1 - 3m_1r})$. To prove $\modelensemble$ is a robust PAC learner for any $\epsilon$ and $\delta$, we need to show there exist $m_1$, $r$, $\delta_1$, and $\epsilon_1$ such that $\epsilon \geq  1 - (1 - \delta_1 -  \frac{3\epsilon_1}{1 - 3m_1r})$. 
% % We then have $1 - (1 - \delta_1 -  \frac{2\epsilon_1}{1 - 2m_1r}) \leq \delta_1 + \frac{2\epsilon_1(1 - m_1r)}{1 - 2m_1r} \leq \delta_1 + 2\epsilon_1 +  \frac{2\epsilon_1}{\frac{1}{m_1r} - 2}$. Therefore, let $\epsilon_1 = \frac{\epsilon}{5}$, $\delta_1 = \frac{\epsilon}{5}$ and $r \leq \frac{1}{3m_1}$, $\modelensemble$ is a $r$-robust PAC learner. In this case, we have $\hat{m}_{\cH}(\epsilon, \delta) = m_H(1/5\epsilon, 1/5\epsilon)$.
% % As we assume $r = o(1)$, for every $\lambda$ there exists a constant $N$ such that $r<\lambda$ for every $n \geq N$. Now, let $\lambda = (\epsilon/4-\delta)/m$ and $\epsilon_1 = \frac{1}{4}\epsilon$, we have $\Pr[\modelensemble(x_e) = y_e] \geq \Pr\left[(1 - \epsilon_e)(1 - \delta)(1-mr) \geq 1/2\right] \geq 1 - \Pr[\epsilon_e \geq 1 - \frac{1}{2(1 - mr)(1 - \delta)}] \geq 1 - \frac{1}{2}\epsilon - \frac{1}{2}\epsilon \geq 1 - \epsilon$. For a large enough sample complexity $n$, we will have error smaller than $\epsilon$.
% \end{proof}

% \begin{lemma}
% For an ensemble model $h_e: \{h_1, \dots, h_k \}$, suppose each $h_i$ is trained with ERM on $m$ samples that i.i.d sampled from 
% $n=|S|$ samples and has generalization error $2\epsilon$. The ensemble model is $r$-Point-wise Robust for at least $(1 - 2r - 2\epsilon)|S|$ sample.
% \end{lemma}
% \begin{proof}
% For each model $h_j$, $r$ faction of the data is changed. Therefore, average generalization error is at most $2r+2\epsilon$. There are at least $k(1-2r-2\epsilon)$ fraction of data is correctly predicted. 
% % Therefore, the ensemble model is $r$-Point-wise Robust for at least $(1 - 2r - 2\epsilon)|S|$ sample.
% \end{proof}

% \begin{definition}[Agnostic k-Robust PAC learnability]
% We call a hypothesis class $\cH$ is $r$-strong-robust agnostic PAC learnable if there exist a function $\tilde{m}_{\cH}: (0,1)^2 \rightarrow \cN$ and a learning algorithm $\Learn$ with the following property: For every $ \epsilon, \delta \in (0, 1)$, every distribution $\cD$ over $\cX$ and for every labeling function $f: \cX \rightarrow \{0,1\}$,
% % , in the realizable setting, 
% suppose there exists a dataset $\cS$ that has $n \geq \tilde{m}_{\cH}(\epsilon, \delta)$ i.i.d examples from $\cD$ and $f$. An adversary modify $\cS$ to $\cS'$, where $\HD(\cS, \cS') \leq r|n|$ with the knowledge of the learning algorithm $\Learn$ and all the random numbers used by $\Learn$. Then regardless of any given $\cS'$ , algorithm $\Learn$ returns a hypothesis $h$ such that, for over probability $1 - \epsilon - \min_{h'}\loss_{\cD}(h')$ on $\cD$, $h$ is correct with probability of at least $1 - \delta$.
% \label{def:strongrobustagnostic}
% \end{definition}

% \begin{theorem}
% $\cH$ is $r = o(1)$ strong robust agnostic PAC learnable if $\cH$ is PAC learnable. 
% \end{theorem}

% \begin{proof}
% Similarly, we show that majority ensemble model $\modelensemble$ is also $r$-strong-robust agnostic PAC learner.

% Let $K$ denotes the number of sub-models in $K$. Now, suppose the learner $\modelensemble$ first i.i.d. sample $n = Km$ examples and then separate them into $K$ partitions, each partition includes $m$ examples, by giving each example a label of the partition ID. Each sub-learners then train with the partition of its corresponding ID. These sub-learners are independent to each other.

% For each sub-model, by the fundamental theorem of statistical learning, when 
% $m \geq m^{UC}_\cH(\epsilon_1/2, \delta_1)$ (where $m^{UC}_\cH$ is the sample complexity function of uniform convergence on hypothesis set $\cH$), if $h$ is trained with $\cS$, $h$ has probability at least $1-\delta_1$ that generalization loss $\loss_{\cD}(h)$ is at most $\epsilon_1 + \epsilon$, where $\epsilon = \min_{h \in \cH} \loss_{\cD}(h)$ is the minimal generalization loss among the hypothesis set $\cH$. Now, since the adversary tampers $k = rn$ examples, at least $K - k$ partitions are not touched by the adversary. 


% \end{proof}

